Art or Artifice? Large Language Models and the False Promise of Creativity

Researchers have argued that large language models (LLMs) exhibit high-quality writing capabilities from blogs to stories. However, evaluating objectively the creativity of a piece of writing is challenging. Inspired by the Torrance Test of Creative Thinking (TTCT), which measures creativity as a process, we use the Consensual Assessment Technique [3] and propose the Torrance Test of Creative Writing (TTCW) to evaluate creativity as a product. TTCW consists of 14 binary tests organized into the original dimensions of Fluency, Flexibility, Originality, and Elaboration. We recruit 10 creative writers and implement a human assessment of 48 stories written either by professional authors or LLMs using TTCW. Our analysis shows that LLM-generated stories pass 3-10X less TTCW tests than stories written by professionals. In addition, we explore the use of LLMs as assessors to automate the TTCW evaluation, revealing that none of the LLMs positively correlate with the expert assessments.

==> 1-intro.tex <==
\section{Introduction}
\label{sec:intro}

% \textbf{SARAH - - intro paragraph 1 feels a little all over in the way it addresses creativity — I’d suggest making sure you are specific about whether you are discussing person-focused creativity or artifact-focused creativity.  The last sentence about what you are interested in is key — expand that slightly so we know why it’s difficult to use TTCT.
% \\
% paragraph 2 — “complying” is a weird phrasing here — I’m not sure what that means or why you use that to adapt the TCTT
% \\
% overall I think you need a little more context to start out — instead of jumping into defining creativity history, give half a paragraph on why the work you’re about to do matters.
% }\\

As AI-assisted writing gets more and more popular  \cite{AIassistedWriting1, AIassistedWriting2}, especially in the wake of an enormous movement in the writing industry \cite{WGA}, it is rather timely and urgent to evaluate whether LLMs have the abilities to generate creative content and whether they can assess and critique the creativity of an existing piece.Creativity is often difficult to evaluate because it is a complex, multifaceted concept that is deeply subjective, contextual, and hard to judge objectively. Several empirical studies have been conducted in psychology and cognitive science on the processes through which creativity occurs \cite{kurtzberg2005feeling,cropley2000defining,silvia2008assessing}. Interpretation of the results has led to several possible explanations of the sources and methods of creativity. Eminent psychologist J. P. Guilford drew a distinction between convergent and divergent thinking \cite{guilford1967nature}. Convergent thinking involves aiming for a single, correct solution to a problem, whereas divergent thinking involves the creative generation of multiple answers to a set problem. Divergent thinking is sometimes used as a synonym for creativity in psychology literature or is considered the necessary precursor to creativity \cite{RUNCO2011400}. 

Built on J.P. Guilford's work Ellis Paul Torrance devised one of the widely accepted tests of creativity, \textit{Torrance Tests of Creative Thinking (TTCT)} \cite{torrance1966torrance}, which originally involved simple tests of divergent thinking and other problem-solving skills. Prior work has argued that creative writing constitutes a promising topic for an interdisciplinary conversation about creativity \cite{Doyle1998TheWT}. One of the popular frameworks for Creativity evaluation, TTCT -- typically involves two parts: Verbal and Figural -- measures creativity as a process by testing participants' abilities in dealing with unusual uses of objects, specific situations, or impossibilities. We are however interested in measuring creativity as a product within the realm of short story writing making it difficult to directly rely on TTCT \cite {baer2009assessing}.

In the field of Computer Science, recent work has shown the promise of LLMs in creative writing tasks \cite{mirowski2023cowriting,yang2022re3,lee2022coauthor}, without reaching a consensus on how to evaluate creative writing. Towards this, we design a framework particularly aimed at evaluating creativity as a product by adapting prior work on the evaluation of creativity as a process (Section \ref{design} Design Principle 1 and 2). One of the popular methods for Creativity Evaluation called the \textit{Consensual Assessment Technique} \cite{amabile1982social} states that the most valid assessment of the creativity of an idea or creation in any field is the collective judgment of experts in that field. Similarly in this work, we first collaborate with 8 creative writing experts to collect creativity measures for the evaluation of short fictional stories. 

The evaluation protocol we propose, the Torrance Tests for Creative Writing (TTCW), consists of 14 binary tests organized into the original Torrance dimensions of \textit{Fluency, Flexibility, Originality} and \textit{Elaboration}. In Section~\ref{sec:approach}, we go over the process we followed to create the TTCW by collecting insights from expert creative writers and consolidating them into individual tests. To empirically validate the TTCW as an evaluation method, we create in Section~\ref{sec:data} a benchmark consisting of 48 short stories (12 stories written by professionals, and 36 by various modern LLMs, with 1400 words in average per story). We recruit a new set of 10 experts, again in compliance with CAT, to administer the TTCW on each story, collecting 3 evaluations per story. Based on a total of 2,000+ expert-administered tests, our findings reveal that experts reach moderate agreement on average (Fleiss Kappa $[0.4-0.6]$) across the 14 TTCW tests, and reach strong agreement when considering the aggregated tests (Pearson correlation $0.69$). This confirms the validity of our TTCW for the evaluation of creativity in fictional short stories.

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/CHI_pipeline.pdf}
\caption{\label{pipeline}Pipeline showing the construction of TTCW and evaluation of short stories using the TTCW framework}
\end{figure*}

The analysis of the conducted tests reveals that the 12 expert-written stories pass an average of 84.7\% of the tests, confirming that although an expert story must not pass all tests to be deemed creative, experienced writers typically produce artifacts that pass the majority of the tests. In comparison, LLM-generated stories pass many fewer tests on average, from 9\% for ChatGPT-generated~\footnote{\url{https://openai.com}} stories, up to 30\% for Claude-generated~\footnote{\url{https://www.anthropic.com}} stories. In other words, LLM-generated stories are three to ten times less likely to pass individual TTCW tests compared to expert-written stories, revealing a wide gap in the evaluated creativity of LLM-generated content. Besides the general gap, the granularity of the TTCW reveals that individual LLMs differ in abilities, with GPT4 more likely to pass tests associated with Originality, and Claude V1.3 more likely to pass tests in Fluency, Flexibility and Elaboration.

Prior work has argued that even though LLMs might not be able to produce creative content in an end-to-end fashion, they might be utilized in providing feedback to authors during their writing process \cite{ippolito2022creative}. To this effect, we explore in Section ~\ref{sec:llmeval} whether LLMs can administer individual TTCW tests individually, by expanding each test into a detailed prompt, and measuring whether LLM assessments correlate with collected expert judgments. Our analysis reveals that for the most part, LLMs are not capable of administering the TTCW tests, as the three LLMs we experiment with -- ChatGPT, GPT4, and Claude 1.3 -- achieve correlations with experts that are close to zero.

In summary, our work makes the following contributions:
\begin{itemize}
    \item We adapt the Torrance Test for Creative Thinking (TTCT), a framework for evaluating creativity as a process, and align it for the evaluation of creativity as a product particularly focusing on short stories. We design 14 tests called the \textit{Torrance Test for Creative Writing (TTCW)} based on the four original Torrance dimensions of Fluency. Flexibility, Originality, and Elaboration,
    \item We experimentally validate the TTCW through a large-scale assessment of 48 stories involving 10 participants with expertise in creative writing, finding that they reach moderate agreement when administering individual tests, and strong agreement when evaluating all tests in aggregate.
    \item We study the abilities of LLMs to generate stories that pass/fail the TTCW tests and their ability to reliably assess the creativity of stories following the TTCW framework through correlation with human judgments. Our findings show that LLM-generated stories are three to ten times less likely to pass TTCW tests compared to expert-written stories, as well as the fact that current state-of-the-art LLMs are not yet capable of reproducing expert assessments when administering TTCW tests. To enable future research in this fast-evolving domain, we plan to release the large-scale annotation of 2,000+ TTCW assessments, each accompanied with a natural language expert explanation. 
    \item Finally, we discuss how creative writing experts can distinguish between AI v.s. human written stories and how future work can use our evaluation framework for building rich interactive writing support tools.
\end{itemize}


==> figures/analysis.tex <==
% \begin{figure*}
%     \centering
%     \begin{subfigure}[b]{1.0\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/GPT3.5.pdf}
%          \caption{Binary judgements across 48 stories from GPT3.5 on 14 tests}
%          \label{fig:GPT3.5YesNo}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{1.0\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/GPT4.pdf}
%         \caption{Binary judgements across 48 stories from GPT4 on 14 tests}
%         \label{fig:categories}
%     \end{subfigure}
%     \label{fig:GPT4YesNo}
%       \begin{subfigure}[b]{1.0\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Claude.pdf}
%         \caption{Binary judgements across 48 stories from Claude on 14 tests}
%         \label{fig:categories}
%     \end{subfigure}
%     \label{fig:ClaudeYesNo}
% \end{figure*}


==> figures/approach.tex <==
\section{Designing Tests for Creative Writing} \label{sec:approach}
\subsection{Rethinking Torrance Test of Creative Thinking}
Built on J.P. Guilford's work and created by Ellis Paul Torrance, the Torrance Tests of Creative Thinking, a test of creativity, originally involved simple tests of divergent thinking and other problem-solving skills, which were scored on four scales:

\begin{figure*}
\centering
\small
\includegraphics[width=0.8\textwidth]{figures/interface.png}
\caption{\label{fig:interface}Interface to collect Creativity measurements across the four-dimensional analytical framework derived from the Torrance Test of Creative Thinking}
\end{figure*}

\begin{itemize}
    \item Fluency. The total number of interpretable, meaningful, and relevant ideas generated in response to the stimulus.
    \item  Flexibility. The number of different categories of relevant responses.
    \item Originality. The statistical rarity of the responses.
    \item Elaboration. The amount of detail in the responses.
\end{itemize}

While prior work \cite{10.1145/3313831.3376495,10.1145/1978942.1979048,Beketayev2016ScoringDT} has utilized Torrance Test of Creative Thinking in other domains, it hasn't been used to evaluate creative writing. Even though the overall dimensions are generalizable across various forms of art, there are measures specific to creative writing along these dimensions that require the existing definitions to be revised and expanded. For this we recruit experts in creative writing. 

\subsection{Participant Recruitment}
In prior work \cite{gero2023social} has argued that the definition of an ‘expert’ or ‘amateur’ creative writer is difficult in a field that has unclear professional delineations.Though it could be feasible to enlist individuals self-identifying as creative professionals, our requirements necessitated the procurement of participants possessing an intricate and analytical comprehension of the creative writing process. Accordingly, we delimited our participant acquisition to those possessing either a structured educational background in creative writing (for instance, a Master of Fine Arts in Creative Writing), traditionally published authors \footnote{We do not recruit self-published authors}, or lecturers/professors instructing Fiction Writing at the university level.Our recruitment thus resulted in participants who have published novels with leading publishing giants, students enrolled in top MFA programs in the United States, University professors teaching Fiction Writing and screenwriters from prime-time network. Participants were recruited through \textit{User Interviews} (a professional freelancing website) and were paid 70\$ for a taking part in an hour long survey. Table \ref{surveyprof} shows our recruited participants.

\begin{table}[!ht]
\centering
\small
\def\arraystretch{1.35}
\parbox{.45\linewidth}{\begin{tabular}{ll}
\hline
ID & Profession                  \\ \hline
W1 & Professor of Creative Writing \\ \hline
W2 & Professor of Creative Writing \\ \hline
W3 & Lecturer in Creative Writing  \\ \hline
W4 & MFA Fiction Student           \\ \hline
W5 & MFA Fiction Student           \\ \hline
W6 & MFA Fiction Student           \\ \hline
W7 & Author                        \\ \hline
W8 & ScreenWriter                  \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{surveyprof}Background of Participants recruited for collecting judgements about Creativity across the dimensions of Torrance Test}
}
\quad\quad\quad\quad
\parbox{.45\linewidth}
{\begin{tabular}{ll}
\hline
Cluster & Participants                  \\ \hline
Narrative Pacing & W4,W6,W7 \\ \hline
\begin{tabular}[c]{@{}l@{}}Understandability\\ \& Coherence\end{tabular}  & W3,W7 \\ \hline
\begin{tabular}[c]{@{}l@{}}Language Proficiency\\ \& Literary Devices\end{tabular}  & W4,W2  \\ \hline
Narrative Ending & W3           \\ \hline
Scene vs Summary & W2,W5,W8          \\ \hline\hline
Structural Flexibility & W3,W7,W8           \\ \hline
Perspective \& Voice Flexibility & W3,W6                        \\ \hline
Emotional Flexibility & W3                  \\ \hline\hline
Originality in Theme/Content & W3                  \\ \hline
Originality in Thought & W1,W2,W3,W5,W7                  \\ \hline
Originality in Form/Structure & W2,W4                  \\ \hline\hline
World Building \& Setting & W2,W6                  \\ \hline
Rhetorical Complexity & W3,W4                  \\ \hline
Character Development & W2,W3,W4,W5,W7,W8                  \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{testsource}Background of Participants recruited for collecting judgements about Creativity across the dimensions of Torrance Test}}
\vspace{-5ex}
\end{table}


\subsection{Collecting Creativity Measures}

\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.5}
\begin{tabular}{|l|l|l|}
\hline
\multirow{5}{*}{Fluency}     & Narrative Pacing                                                                   & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Does the manipulation of time in terms of compression or stretching\\ feel appropriate and balanced?\end{tabular}}}                                                                                                    \\ \cline{2-3} 
                             & Scene vs Exposition                                                                & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Does the story display an awareness and insight into the balance \\ between scene and summary/exposition?\end{tabular}}}                                                                                               \\ \cline{2-3} 
                             & \begin{tabular}[c]{@{}l@{}}Language Proficiency \&\\ Literary Devices\end{tabular} & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Does the story make sophisticated use of idiom or metaphor or\\ literary allusion?\end{tabular}}}                                                                                                                     \\ \cline{2-3} 
                             & Narrative Ending                                                                   & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Does the end of the story feel natural and earned, as opposed to \\ arbitrary or abrupt?\end{tabular}}}                                                                                                               \\ \cline{2-3} 
                             & \begin{tabular}[c]{@{}l@{}}Understandability \&\\ Coherence\end{tabular}           & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Do the different elements of the story work together to form a \\ unified, engaging, and satisfying whole?\end{tabular}}}                                                                                              \\ \hline\hline
\multirow{3}{*}{Flexibility} & \begin{tabular}[c]{@{}l@{}}Perspective \& Voice \\ Flexibility\end{tabular}        & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Does the story provide diverse perspectives, and if there are unlikeable\\ characters, are their perspectives presented convincingly and accurately?\end{tabular}}}                                                    \\ \cline{2-3} 
                             & Emotional Flexibility                                                              & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Does the story achieve a good balance between interiority and exteriority, \\ in a way that feels emotionally flexible?\end{tabular}}}                                                                                 \\ \cline{2-3} 
                             & Structural Flexibility                                                             & \textit{\textbf{Does the story contain turns that are both surprising and appropriate?}}                                                                                                                                                                          \\ \hline\hline
\multirow{3}{*}{Originality} & Originality in Thought                                 & \textit{\textbf{Is the story an original piece of writing without any cliches?}}                                                                                                                                                                                  \\ \cline{2-3} 
                             & \begin{tabular}[c]{@{}l@{}}Originality in Theme \\ \& Content\end{tabular}                                      & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Will an average reader of this story obtain a unique and original idea \\ from reading it?\end{tabular}}}                                                                                                              \\ \cline{2-3} 
                             & \begin{tabular}[c]{@{}l@{}}Originality in Form/ \\ Structure\end{tabular}          & \textit{\textbf{Does the story show originality in its form and/or structure?}}                                                                                                                                                                                   \\ \hline\hline
\multirow{3}{*}{Elaboration} & \begin{tabular}[c]{@{}l@{}}World Building \& \\ Setting\end{tabular}               & \textit{\textbf{Does the writer make the fictional world believable at the sensory level?}}                                                                                                                                                                      \\ \cline{2-3} 
                             & Character Development                                                              & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Does each character in the story feel developed at the appropriate complexity\\ level, ensuring that no character feels like they are present simply to satisfy\\ a plot requirement?\end{tabular}}} \\ \cline{2-3} 
                             & Rhetorical Complexity                                                              & \textit{\textbf{Does the story operate at multiple 'levels' of meaning (surface and subtext)?}}                                                                                                                                                                  \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{CreativityTest} Clusters with individual questions to empirically measure creativity across the four dimensions of Torrance Test}
\end{table*}

Following participant enlistment, we explained our objective aimed at assessing creativity in any piece fiction or creative non-fiction, utilizing the four-dimensional analytical framework derived from the Torrance Test of Creative Thinking. Explicit instructions were provided requesting participants to concisely articulate methodologies employed in gauging creativity across these dimensions. In formulating their responses, participants were exhorted to adopt an empirical mindset and eschew abstract or indeterminate terminologies that lack quantifiable attributes. Figure \ref{fig:interface} shows our interface to collect these responses. For each dimension we allowed our participants to state up to 5 measures. We received a total 126 measures from 8 participants across the 4 dimensions. On average each participant provided with 16 measures, 4 for each dimension of creativity.

The measures derived from the involved participants exhibited a considerable degree of semantic congruence. To consolidate these measures from them we prompt GPT-4 \cite{OpenAI2023GPT4TR} to distribute them into individual clusters, each of which encapsulates a generalized representation of a given measure.Each individual cluster was subsequently subjected to a rigorous review by a panel of four domain-specific experts to confirm both the validity of their classification and the comprehensiveness of the represented measures.Measures that could not be quantified empirically at all were discarded.In total we ended up with 14 distinct clusters with 5 representative measures for Fluency and 3 representative measures each for Flexibility, Originality and Elaboration.Some of these measures for creativity came from an individual participant while some measures were uniformly suggested by multiple participants as can be seen in Table \ref{testsource}.

\section{What do these measures tell about Creative Writing?}
Table \ref{CreativityTest} shows the representative measure from each individual cluster across the four dimensions of Creativity.These measures test several aspect of creative writing ranging from originality of thought to well-rounded character development.
\subsection{Fluency}
Compared with both reading and speaking fluency, writing fluency has always been traditionally harder to define \cite{abdel2013we}.Our 5 measures across this dimensions each look at individual aspects of creative writing. 
\subsubsection{Narrative Pacing} 
This measure refers to the manipulation of time in storytelling for dramatic effect. Essentially, it's about controlling the perceived speed and rhythm at which a story unfolds.A skilled writer can manipulate the relationship between these two to affect the pacing of the narrative, either speeding it up (compression) or slowing it down (stretching). This technique plays a crucial role in shaping the reader's experience and engagement with the story. 
\footnote{\url{https://www.writingclasses.com/toolbox/articles/stretching-and-shrinking-time}}
\subsubsection{Scene vs Exposition}
A 'Scene' is a moment in the story that is dramatized in real-time often featuring character interaction, dialogue, and action while 'Exposition', on the other hand, involves summarizing events or providing information like character history, setting details, or prior events. The right balance between scene and summary/exposition can vary depending on the story, but in general, it's essential for maintaining a good pace, keeping the reader engaged, and delivering necessary information \cite{burroway2019writing}. 
\footnote{\url{https://creativenonfiction.org/syllabus/scene-summary/}}
\subsubsection{Language Proficiency \& Literary Devices} 
Eminent novelist Milan Kundera said ``\textit{Metaphors are not to be trifled with. A single metaphor can give birth to love.}". Sophisticated use of literary allusion or figurative language such as metaphor/idioms often add depth, interest, and nuanced meaning to any creative writing. It allows for a richer reading experience, where the literal events are imbued with deeper symbolic or thematic significance. 
\subsubsection{Narrative Ending}
In her New Yorker essay ``On Bad Endings" \cite{BadEndings} Joan Accocela writes 
            \begin{quote}
                \centering
                ``Another possibility is that the author just gets tired. I review a lot of books, many of them non-fiction. Again and again, the last chapters are hasty and dull. `I’ve worked hard enough,' the author seems to be saying. `My advance wasn’t much. I already have the idea for my next book. Get me out of here.'"
            \end{quote}
If the writer ends the piece simply because they are ``tired of writing", the conclusion might feel abrupt, disjointed, or unfulfilling to the reader. This is one of the important factors of creative writing fluency.A strong ending offers a sense of closure, ties up the central conflicts or questions of the story, and generally leaves the reader feeling that the narrative journey was worthwhile and complete.
\subsubsection{Understandability \& Coherence}
Narrative coherence is the degree to which a story makes sense  \footnote{https://en.wikipedia.org/wiki/Narrative\_paradigm}.A well-crafted story usually follows a logical path, where the events in the beginning set up the middle, which then logically leads to the end. Every scene, character action, and piece of dialogue should serve the story and propel it forward. Well-written stories have an underlying unity that binds the elements together. The themes, plotlines, character arcs, and other elements of the story interweave to create a harmonious whole. A story with `disorder' might feel disjointed, with characters, scenes, etc that don't connect or contribute to the overall narrative.

\subsection{Flexibility}
Flexibility is often referred to as the ability to look at something from a different angle or point of view. In the context of creative writing our participants agreed on 3 distinct measures of Flexibility
\subsubsection{Perspective \& Voice Flexibility}
An \textit{omniscient} narrator is the all-knowing voice in a story that can convincingly and accurately depict a wide range of character viewpoints, including those of characters who may be morally ambiguous, difficult, or otherwise unappealing. This can also potentially involve diving into the mindset of characters who may act or think in ways that the reader, or even the writer, finds objectionable or repugnant.As stated in \cite{friedman1955point} an omniscient narrator enhances a sense of reliability or truth within literary works since readers are given deeper insights into many characters. The multiple viewpoints feel more objective because readers have access to multiple interpretations of events and can thus decide how they feel about each character’s perspective.
\subsubsection{Emotional Flexibility}
Emotional flexibility is asking whether the piece of writing effectively balances action and introspection, and if it portrays a broad and realistic spectrum of emotions. \textit{Exteriority} refers to the observable actions, behaviors, or dialogue of a character, and the physical or visible aspects of the setting, plot, and conflicts.\textit{Interiority}, on the other hand, pertains to the inner life of a character — their thoughts, feelings, memories, and subjective experiences. A balance between these two aspects is crucial in creating well-rounded characters and compelling narratives. As stated in \cite{campe2014rethinking} if a story is too heavy on exteriority, it may feel shallow or lack emotional depth. If it leans too much on interiority, it could become overly introspective and potentially lose the momentum of the plot.
\subsubsection{Structural Flexibility}
A good piece of creative writing often has plot twists, character developments, or thematic revelations that surprise the reader, subverting their expectations in a thrilling way. It's about keeping readers engaged and curious, never fully knowing what's going to happen next. However despite the surprises and twists, the turns in the story must also make sense within the established context of the story's universe, its characters, and its themes. This means that even though an event might be surprising, it should feel appropriate or fitting in hindsight. It shouldn't feel like the writer has broken the rules they've set up, or made a character behave inconsistently without reason, simply for the sake of shock value.
\subsection{Originality}
Creative writing requires originality, or the ability to generate unique ideas \cite{ward1999creative}. Originality can conveyed in several ways. Our participants suggested three unique ways in which they look for originality in creative writing.
\subsubsection{Originality in Theme and Content}
In his book ``Literature and the Brain" well-known literary critic and scholar Norman Holland discusses how stories stimulate the mind and impact readers \cite{holland2009literature}. A good story that offers a deeper understanding of human nature, cultural insights,unique viewpoints, or even the exploration of new ideas and themes has a lasting impact on its reader and society .It is meant to entertain, inform, provoke thought, challenge beliefs, provide comfort, or raise awareness on specific issues.In ``Poetic Justice", prominent philosophers Martha Nussbaum explores how the literary imagination is an essential ingredient of public discourse and a democratic society \cite{nussbaum1997poetic}.As such originality in theme and content is an important measure of creative writing.
\subsubsection{Originality in Thought}
A cliche is an idea, expression, character, or plot that has been overused to the point of losing its original meaning or impact \cite{fountain2012cliches}. They often become predictable and uninteresting for the reader.In his book \cite{clark2008writing} eminent American writer, editor, and a writing coach: Roy Peter Clark advised writers to strictly avoid cliches because they often indicate a lack of original thought or laziness in language use.Originality suggests that the piece isn't cliche.
\subsubsection{Originality in Form/Structure}
In his book \cite{boardman1992narrative} Michael M. Boardman discusses how innovation in narrative structure can serve ideological purposes and challenge conventional narrative forms. Frederic Jameson  highlighted the complexities of postmodern literature, where the blurring of genres and innovation in form and structure was a key characteristic\cite{jameson1991postmodernism}. Originality in form/structure has also been accomplished by unconventional use of format, genre or plot structure.For instance, the Pulitzer winning book \textit{The Color Purple} from Alice Walker is told through a series of letters written by the protagonist. Neil Gaiman's \textit{American Gods} on the other hand combines elements of fantasy, mystery, and mythic fiction in unexpected ways. \textit{The Sound and the Fury} by William Faulkner deviates from the traditional plot structure by presenting a narrative that unfolds through the stream of consciousness of different characters. The goal of originality in form or structure is often to provide a fresh reader experience, challenge conventional reading expectations, or to create a deeper or more complex exploration of the story's themes.
\subsection{Elaboration}
\subsubsection{World Building and Setting}
American poet and memoirist Mark Doty discusses the importance of create a vivid, immersive reality at the sensory level through the use of detailed, evocative description \cite{doty2014art84794531}.An effective writer often uses sensory details to paint a detailed picture of the story's environment, making it feel tangible and real to the reader.For example, describing the specific colors and shapes in a scene, the sounds that fill a space, the textures and temperatures that a character comes into contact with, the flavors of the food they eat, or the scents that fill the air, can all contribute to creating a sensory-rich and believable world.By stimulating the reader's senses, the writer can make the reader feel as though they're experiencing the events of the story firsthand. This level of detail contributes to the believability of the world, even if it's a completely fictional or fantastical setting. It helps the reader to suspend disbelief and become more deeply invested in the narrative.
\subsubsection{Character Development}
A 'flat character' is typically a minor character who is not thoroughly developed or who does not undergo significant change or growth throughout the story. They often embody or represent a single trait or idea, and they're only used to advance the plot or highlight certain qualities in other characters. A 'complex character' on the other hand also known as a round character, has depth in feelings and passions, has a variety of traits of a real human being, and evolves over time. They have their strengths, weaknesses, and they learn from their experiences. \cite{forster1927aspects,fishelov1990types,currie1990nature} highlights that any creative piece of fiction or non-fiction tend to be more engaging to the reader when authors can take a character who initially appears to be one-dimensional or stereotypical (flat) and add depth to them, as it mirror the complexity of real people.
\subsubsection{Rhetorical Complexity}
In Ernest Hemingway's short story "Hills Like White Elephants," the couple's conversation about seemingly unrelated topics implies a much deeper and more serious discussion about an abortion. Their actual dialogue never directly addresses this issue, but it's heavily suggested through what's left unsaid — the subtext. Effective writing often operates on both surface and subtext levels. The surface text keeps the reader engaged with the plot and characters, while the subtext provides depth, complexity, and additional layers of interpretation, contributing to a richer and more rewarding reading experience \cite{kochis2007baxter,phelan1996narrative}.



==> figures/data.tex <==
\section{Data Design for creative writing evaluation}

\begin{table*}
\def\arraystretch{1.35}
\small
\centering
\begin{tabular}{|l|l|}
\hline
Story                                    & Plot                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\href{https://www.newyorker.com/books/flash-fiction/a-triangle}{A Triangle}                               & \begin{tabular}[c]{@{}l@{}}An observer becomes entranced by a seemingly ordinary couple on the street, follows them home,\\ and then watches them from  outside in the rising floodwaters, drawing an eerie connection \\ between the woman and a discarded, burned chair they'd noticed earlier.\end{tabular}                                                                                                                                                                    \\ \hline\hline
\href{https://www.newyorker.com/books/flash-fiction/barbara-detroit-1966}{Barbara,Detroit,1996 }                    & \begin{tabular}[c]{@{}l@{}}On February 12, 1966, a heavily pregnant woman named Barbara experienced a shocking incident in her\\ synagogue in Southfield, Detroit, where a young man shot and killed the renowned Rabbi Adler before\\ turning the gun on himself, and though Barbara tried to reach the shooter, she was swept away by the\\ fleeing crowd.\end{tabular}                                                                              \\ \hline\hline
\href{https://www.newyorker.com/books/flash-fiction/beyond-nature}{Beyond Nature}                           & \begin{tabular}[c]{@{}l@{}}A solitary man walking in a remote mountainous region comes across a car crash, and stays by the side\\ of the lifeless female victim, narrating stories of his past and reflecting on the impermanence of \\events and life itself, while awaiting emergency services amidst the looming presence of wilderness.\end{tabular}                                                                                                                \\ \hline\hline
\href{https://www.newyorker.com/books/flash-fiction/certain-european-movies}{Certain European Movies}                  & \begin{tabular}[c]{@{}l@{}}Two individuals, who are at a residency together, navigate the complexity of their ephemeral relationship \\during their final beach trip, framed by misadventures, subtle tensions, unspoken desires, and \\looming departures.\end{tabular}                                                                                                                                                                                   \\ \hline\hline
\href{https://www.newyorker.com/books/flash-fiction/keys}{Keys}                                     & \begin{tabular}[c]{@{}l@{}}Daniel, struggling with recurring dreams of his ex-wife Rachel and a mysterious unused flat, eventually \\discusses them with his current partner Isabel, sparking various reflections and conversations about their\\ past relationships, until a real-life discovery of old keys triggers a nostalgic memory and helps him find a\\ way to reconnect with his present relationship through canoeing.\end{tabular}                                     \\ \hline\hline
\href{https://www.newyorker.com/books/flash-fiction/listening-for-the-click}{Listening For the Click}                  & \begin{tabular}[c]{@{}l@{}}Navigating a complex social landscape, the protagonist experiences a series of complex relationships \\and emotional turmoil in a student  environment, and engages in self-discovery and self-reflection as she\\ interacts with the characters Carl, Martin, Lizzy, and Johan, resulting in a journey of introspection, betrayal,\\ love, and personal growth.\end{tabular}                                                          \\ \hline\hline
\href{https://www.newyorker.com/magazine/2023/05/15/maintenance-hvidovre-fiction-olga-ravn}{Maintenance, Hvidovre}                   & \begin{tabular}[c]{@{}l@{}}A woman experiences a disorienting night in a maternity ward where she encounters other similarly \\disoriented new mothers, leading to an uncanny mix-up where she leaves the hospital with a baby that she \\realizes is not her own, yet accepts the situation with an inexplicable sense of happiness.\end{tabular}                                                                                                  \\ \hline\hline
\href{https://www.newyorker.com/magazine/2022/11/14/returns}{Returns}                                  & \begin{tabular}[c]{@{}l@{}}The narrator visits their elderly mother in her small town, spending a day with her that is filled with \\nostalgia, conversation, and old habits, only to return a month later after her hospitalization due to\\ a sunstroke, finding remnants of their last visit.\end{tabular}                                                                                                                                                                      \\ \hline\hline
\href{https://www.newyorker.com/books/flash-fiction/the-facade-renovation-thats-going-well}{\begin{tabular}[c]{@{}l@{}}The Facade Renovation That’s \\Going Well\end{tabular}} & \begin{tabular}[c]{@{}l@{}}An academic faculty housed in a building with a critical waterproofing layer missing experiences a series\\ of disruptive and problematic construction repairs, causing tension, inconvenience, and health concerns\\ among the tenants, but ultimately leading to resignation and endurance in hopes of better future\\ circumstances.\end{tabular}                                                        \\ \hline\hline
\href{https://www.newyorker.com/books/flash-fiction/the-kingdom-that-failed}{The Kingdom That Failed}                  & \begin{tabular}[c]{@{}l@{}}The narrator recounts their college friendship with the seemingly flawless Q, and after a decade apart, \\they accidentally cross paths at a pool, where the narrator anonymously observes Q's failed attempt to \\let down a woman about a work-related issue, demonstrating that Q, too, has his share of difficulties.\end{tabular}                                                                                                \\ \hline\hline
\href{https://www.newyorker.com/magazine/2022/06/13/trash }{Trash}                                    & \begin{tabular}[c]{@{}l@{}}A woman unexpectedly marries the son of a successful, ambitious woman named Miss Emily, finding both \\acceptance and critique from her mother-in-law as she navigates this new relationship and confronts the \\stark contrasts between her  former life as a supermarket cashier and her new life as part of a well-off family.\end{tabular}                                                                                                            \\ \hline\hline
\href{https://www.newyorker.com/culture/personal-history/the-last-dance-with-my-dad}{The Last Dance with my Dad}               & \begin{tabular}[c]{@{}l@{}}A young teenager recounts her experiences of fitting into her father's gay lifestyle, highlighted by a\\ seven-day cruise with hundreds of gay men, where she  experienced acceptance and connection, had her\\ first genuine interaction with a  boy, and shared a last dance with her terminally ill father.\end{tabular}                                                                                                       \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{teststories} Expert-written short stories from the New Yorker along with their human-verified GPT4 generated summary as plots that are included as part of our test data for Creativity Evaluation}
\end{table*}


Large Language models have been shown to automatically generate long and coherent stories \cite{yang2022doc,yang2022re3} as well as act as collaborators for creative writing \cite{yuan2022wordcraft,ippolito2022creative,mirowski2023cowriting}. However, there have been fewer studies showing how LLM-generated stories differ from expert written stories on metrics that are more fine-grained and objective.Our investigation involves an analysis of a dozen narratives authored by humans, as detailed in Table \ref{teststories}, extracted from The New Yorker. These narratives span a variety of esteemed authors, ranging from \textit{Haruki Murakami} to Nobel laureate \textit{Annie Ernaux}. The protocol for our human assessment incorporates two primary components: 

\begin{itemize}[leftmargin=*]
    \itemsep0em 
    \item Absolute evaluation of creative writing, disregarding whether it has been composed by a human or a LLM
    \item Relative evaluation for discerning whether a story has been produced by a human or an LLM( Turing Test).
\end{itemize}


\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/datapipeline.pdf}
\caption{\label{datapipeline}Pipeline showing how our test set is created for evaluation. For each human-written original NewYorker story, we generate 3 stories from one LLM each, based on the plot of the original story. The plot is a single-sentence summary of the original story automatically generated by GPT-4 and verified by humans.}
\end{figure*}


In order to allow relative evaluation each human-authored narrative is summarized into a single-sentence plot, which is further verified by human evaluators. We then prompt three LLMs: GPT3.5, GPT4, and Claude, to generate a story conditioned on this plot summary. This yields a total of 48 short narratives for absolute evaluation (12 human written; 36 LLM written). Following this, we assign four stories centered around a single plot (one human-authored versus three LLM-authored) to a singular cluster, culminating in a total of 12 clusters. The methodology for creating an individual cluster is illustrated in Figure \ref{datapipeline}. The decision to employ human-authored plot summaries to prompt the LLMs is informed by the recognized shortfall of LLMs in their ability to devise original plotlines, as highlighted in previous research \cite{ippolito2022creative}. Furthermore, the utilization of multiple stories derived from the same plot enables experts to concentrate specifically on the human aspects of creative writing, and enhances their capacity to distinguish human-generated content from AI-produced ones.

In our quest to prevent straightforward parameters from differentiating between stories penned by human authors versus those produced by artificial intelligence (AI), we implemented strategies to ensure comparable story lengths across both classes. Initial experimentation revealed a notable discrepancy: Large Language Models (LLMs), when instructed to generate narratives of a predetermined word count, consistently underperformed, resulting in stories that were invariably more concise than intended. To address this inconsistency, we employed an iterative mechanism, prompting the LLM to iteratively rewrite the initial story until the divergence in word count between the AI-generated and human-composed story was less than 200 for every cluster. Table \ref{promptstory} (Row1) shows the original story prompt, while (Row2) illustrates the subsequent instruction to rewrite the story. We start the iterative process by prompting the LLM to expand the initially generated story. This cycle continued until the narrative length reached the pre-specified threshold or when the iteration count exceeded twenty ($loop\_count > $20). This methodology ensured the creation of AI-written stories with length characteristics more akin to those produced by human authors.

\begin{figure*}
\small
\centering
\includegraphics[width=\textwidth]{figures/length.png}
\caption{\label{length} Distribution of word count amongst the stories in our test set}
\end{figure*}


\begin{table}[]
\centering
\small
\def\arraystretch{1.35}
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Write a New Yorker-style story given the plot below. Make sure it is atleast \textbf{\color{blue}\{\{word\_count\}\}} words. Directly start with the\\ story, do not say things like `Here's the story {[}...{]}:\end{tabular}                                                                                                                                                                                            \\ \hline\hline
\begin{tabular}[c]{@{}l@{}}You wrote the story I gave you below. I requested a story with \textbf{\color{blue}\{\{word\_count\}\}} words, but the story only has\\ \textbf{\color{blue}\{\{current\_word\_count\}\}} words. Can you rewrite the story to make it longer, and closer to the \textbf{\color{blue}\{\{word\_count\}\}} word target\\ I gave you. Directly start with the story, do not say things like `Here's the story {[}...{]}:`\\ \\ Current story: \{\{story\}\}\end{tabular} \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{promptstory}Prompt to write the initial story (Row1) vs Prompt to rewrite the initial story to be longer. word\_count represents the number of words in the human written story on a given plot (P) while current\_word\_count represents the number of words in the LLM generated story on the same plot (P)}
\vspace{-7ex}
\end{table}

%     
%     \begin{subfigure}[b]{1.0\textwidth}
%          \centering
%          

==> figures/evaluation.tex <==
\section{Evaluation Protocol}
As mentioned earlier our evaluation protocol focuses on the absolute evaluation of the 48 stories on each of the 14 questions shown in Table \ref{CreativityTest} as well as a relative evaluation of 12 clusters for discerning whether a story on the same plot within an individual cluster has been produced by a human or an LLM( Turing Test).
\subsection{Absolute Evaluation}
\subsubsection{Absolute Evaluation with LLMs}
In prior work, \cite{gao2023human} has demonstrated the effectiveness of GPT3.5 over automated metrics in summarization evaluation.\cite{liu2023gpteval} employ the framework of using large language models with chain-of-thoughts (CoT) \cite{wei2022chain} to assess the quality of NLG outputs. Further \cite{rajani2023llm_labels} have shown that GPT4 as an evaluator has a higher correlation with humans for the tasks of brainstorming or creative generation. Following prior work we also use GPT3.5, GPT4, and Claude respectively to provide a verdict (Yes/No) to each of the 14 questions stated in Table \ref{CreativityTest} along with a plausible explanation using Chain-Of-Thought reasoning justifying the answer choice. More details about the evaluation prompts can be found in Section \ref{sec:prompting}. The purpose of our assessment utilizing Large Language Models (LLMs) is not to champion the prospect of a future in which LLMs can adjudicate creativity. Rather, our aim is to decipher the divergence between expert human evaluators and artificial intelligence in comprehending the essence of creativity. We posit that if such models lack the fundamental comprehension of the constituents of creativity, their proficiency in creative writing tasks could be deemed sub-optimal.
\subsubsection{Absolute Evaluation with Creative Writing Experts} A cogent argument posits that the engagement with artistic prose isn't confined solely to specialists, but non-experts also can be competent in assessing imaginative prowess. In prior work, numerous researchers have leveraged annotators sourced from prevalent crowd-sourcing platforms to gauge model outputs, particularly in the domain of creativity. Nevertheless, it is critical to acknowledge that during narrative evaluation trials involving both teachers in English and participants from Amazon Mechanical Turk, the study by \cite{karpinska-etal-2021-perils} exhibited that AMT contributors, even when shortlisted via rigorous eligibility parameters (unlike teachers), struggle to discriminate between model generated text and human-crafted references.In addition, the recent study by \cite{veselovsky2023artificial} highlighted the fact that approximately 33-46\% of crowdworkers on such platforms currently utilize large language models (LLMs) to complete any assigned task.

These complications create the necessity to enlist the expertise of creative writing professionals garnered through \textit{User Interviews}, a prominent freelancing digital platform. A total of eight individuals, adept in creative writing, were enlisted for this endeavor. Five of these experts are associated with the creative writing departments at leading American academic institutions, with considerable experience in conducting undergraduate and graduate level courses. Two of these experts function as literary agents at a top-tier, full-service US literary agency that represents well-recognized authors. The last expert is a Master of Fine Arts student specializing in fiction, who was nominated for the esteemed Pushcart Prize. Similar to LLM's we also ask these experts to provide a verdict (Yes/No) to each of the 14 questions stated in Table \ref{CreativityTest} and subsequently elicit 2-3 sentence explanations justifying the answer.

We conduct this study at a cluster level consisting of 4 stories based on the same plot, however we explicitly ask them to not read all the stories together, as this might potentially confound the ensuing analyses. Participants are explicitly instructed to approach each narrative in an isolated manner, answering a set of 14 targeted queries per individual narrative. All the four stories on the same plot are shuffled randomly based on their source and shared to the experts over a google doc. We use a google form to collect 56 answers and explanations from experts for all the 4 stories within a cluster and pay them 80\$ for a task estimate of 2-2.5 hrs.
\begin{figure*}
    \centering
     \includegraphics[width=\textwidth]{figures/rel.pdf}
    \caption{\label{relev} Relative Evaluation by Creative Writing Experts within a given cluster of four stories}
\end{figure*}
\subsubsection{Relative Evaluation with Creative Writing Experts} After providing verdict on each story inside a particular cluster we ask experts to rank the stories based on their personal preference \cite{ouyang2022training}. This evaluation was also designed with the hope that the most preferred story would also have the highest number of answers to individual questions from the absolute evaluation as `Yes'. Additionally we also ask them to guess the author of each story based on the Turing Test recommendation. We provide them 3 possible author choices to select between \textit{An expert, An amateur, AI} as can be seen in Figure \ref{relev}. This is further useful for us to study if there are certain patterns that leads experts to discriminative between model vs human written stories.

==> figures/intro.tex <==
\section{Introduction}
\label{sec:intro}

Creativity emerges over time in a complex interplay of factors. Human judgments of creativity are often biased by personal tastes, expectations, and hindsight. Scholarly interest in creativity has been found in a number of disciplines, primarily psychology, cognitive sciences and more recently computer science with the advent of large language models. As AI assisted writing gets more and more popular \cite{AIassistedWriting1,AIassistedWriting2} especially in the wake of an enormous movement in the writing industry \cite{WGA} it is rather timely and urgent to evaluate whether large language models understand what it takes to be creative. Creativity is often difficult to evaluate because it is a complex, multifaceted concept that is deeply subjective, contextual, and hard to judge objectively. Several empirical studies have been conducted in psychology and cognitive science of the processes through which creativity occurs.Interpretation of the results of these studies has led to several possible explanations of the sources and methods of creativity. Eminent psychologist J. P. Guilford  drew a distinction between convergent and divergent thinking \cite{guilford1967nature}. Convergent thinking involves aiming for a single, correct solution to a problem, whereas divergent thinking involves creative generation of multiple answers to a set problem. Divergent thinking is sometimes used as a synonym for creativity in psychology literature or is considered the necessary precursor to creativity \cite{RUNCO2011400}. Built on J.P. Guilford's work Ellis Paul Torrance devised one of the widely accepted test of creativity \textit{Torrance Tests of Creative Thinking} \cite{torrance1966torrance} that originally involved simple tests of divergent thinking and other problem-solving skills, which were scored on four scales: \textit{Fluency, Flexibility, Originality, Elaboration}

Creative writing constitutes a promising topic for interdisciplinary conversation \cite{Doyle1998TheWT}. Several researchers have shown the promise of large language models in creative writing tasks \cite{mirowski2023cowriting,yang2022re3,lee2022coauthor} however there has been little consensus in the field of Computer Science on how to empirically evaluate creative writing. To tackle this issue we propose a diagnostic suite of tests that aims to evaluate the creativity in a total of 48 short stories written by both professional writers as well large language models such as GPT3.5, GPT4 and Claude.We construct the foundation of our evaluation through the prism of the \textit{Torrance Tests of Creative Thinking (TTCT)}. Towards this we first we recruit 8 creative writing experts and elicit 4 empirical measures from them across each of the dimensions of \textit{Fluency, Flexibility, Originality} and \textit{Elaboration} in the context of Creative Writing (Section \ref{sec:approach}). These single sentence measures collected from the experts are then subsequently expanded to detailed and quantifiable natural language prompts with the help large language models, followed by careful scrutiny from human experts (Section \ref{sec:prompting}).We then recruit 8 different creative writing experts and ask them alongside leading LLMs such as GPT3.5, GPT4 and Claude to perform the tests described above. The primary objectives of our investigation encompass the resolution of the following research queries:

\begin{itemize}
    \item Can creative writing experts discriminate between stories written by professional writers vs LLMs? 
    \item Are there certain tests for creativity that emerge as discriminative thereby drawing the distinction between good and mediocre writing?
    \item Do LLMs align with expert human judgements across the various dimensions of Creativity and can they provide correct explanation for their judgements?
\end{itemize}




==> figures/promptdesign.tex <==
\section{Converting expert questions to quantifiable Natural language instructions} \label{sec:prompting}

\begin{table*}[!h]
\centering
\small
\def\arraystretch{1.15}
\begin{tabular}{|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Expert \\ Measure\end{tabular}               & Does the writer make the fictional world believable at the sensory level?                                                                                                                                     \\ \hline
\begin{tabular}[c]{@{}l@{}}Expanded\\ Expert\\ Measure (M)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Sensory details pertain to the five senses - sight, sound, touch, taste, and smell. An effective \\ writer can use these elements to paint a detailed picture of the story's environment, making\\ it feel tangible and real to the reader.\\ \\ For example, describing the specific colors and shapes in a scene, the sounds that fill a space,the \\ textures and temperatures that a character comes into contact with, the flavors of the food they \\ eat, or the scents that fill the air, can all contribute to creating a sensory-rich and believable world.\\ \\ By stimulating the reader's senses, the writer can make the reader feel as though they're \\ experiencing the events of the story firsthand.This level of detail contributes to the believability of\\ the world, even if it's a completely fictional or fantastical setting. It helps the reader to suspend\\ disbelief and become more deeply invested in the narrative.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Human\\ Instruction\end{tabular}             & \begin{tabular}[c]{@{}l@{}}\{\{M\}\}\\ \\ Based on the story that you just read, answer the following question.\\ \textit{\color{blue}Does the writer make the fictional world believable at the sensory level?}\end{tabular}                                                                       \\ \hline
\begin{tabular}[c]{@{}l@{}}LLM\\ Instruction\end{tabular}               & \begin{tabular}[c]{@{}l@{}}\{\{M\}\}\\ \\ Given the story above, list out the elements in the story that call to each of the\\ five senses. Then overall, give your reasoning about the question below and give\\ an answer to it between 'Yes' or 'No' only\\ \\ \textit{\color{blue} Q) Does the writer make the fictional world believable at the sensory level?}\end{tabular}                                                                                                                                                                                                                                 \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{prompting}Expert suggested question for World Building and setting (Row1) ; Elucidated prompt designed for other expert humans (Row2); Elucidated quantifiable prompt designed for Large Language Models that elicit Chain of Thought Reasoning(Row3) }
\vspace{-5ex}
\end{table*}

An expert suggested questions for empirically evaluating creative writing might frequently elicit ambiguity in Large Language Models or even other creative writing experts. In order for LLMs or other experts to comprehend the suggested questions in Table \ref{CreativityTest} we attempt at expanding them by adding more details. Recent pre-trained LLMs (e.g., GPT-4 \cite{OpenAI2023GPT4TR} GPT3.5 \cite{ChatGPT}) can engage in fluent, multi-turn conversations out of the box, substantially lowering the data and programming-skill barriers to creating passable conversational user experiences. People can improve LLM outputs by prepending prompts—textual instructions and examples of their desired interactions—to LLM inputs. The prompts steer the model towards generating the desired outputs, raising the ceiling of what conversational UX is achievable for non-AI experts.To elucidate these questions we prompt GPT4 with the following instruction \textit{What do creative experts mean when they say the following: \{\{expert question\}\}}. Once GPT4 gives a response 3 domain experts carefully verify the response and edit it where required in order to convert it into a detailed natural language instruction. Table \ref{prompting} (Row2) shows the human-verified GPT4 elucidated instruction in response to the input prompt.

Prior work \cite{wei2022chain} has shown how generating a \textit{chain of thought} -- a series of intermediate reasoning steps -- significantly improves the ability of large language models to perform complex reasoning. Taking advantage of this we design the prompts for large language models in a slightly different fashion as that of expert humans as can be seen in Table \ref{prompting}. To help the model make an informed decision we first ask it to list out elements specific to any given test such as ``elements in the story that call to each of the five senses" for the World Building and setting test followed by asking it decide overall and then provide its reasoning before choosing an answer between `Yes' or `No'.More examples of Human and LLM instructions for the remaining 13 tests are provided in Appendix \ref{appendix}

==> figures/result.tex <==
\begin{table*}
\small
\centering
\def\arraystretch{1.35}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
      Dimension      & Test & GPT3.5 & GPT4 & Claudev1.3 & Human                         \\ \hline
\multirow{5}{*}{Fluency} & Understandability \& Coherence                                                     &  15.0      & 30.0     &      55.0     &  \textbf{90.0}     \\ \cline{2-6}
 & Narrative Pacing                                                                   &  10.0      &   50.0   &       70.0    &   \textbf{90.0}   \\ \cline{2-6}
 & Scene vs Exposition                                                                &  10.0      &   60.0   &     65.0      &  \textbf{85.0}     \\ \cline{2-6}
 & \begin{tabular}[c]{@{}l@{}}Literary Devices \& Language Proficiency\end{tabular} &   5.0     &   40.0   &     15.0      & \textbf{80.0}      \\ \cline{2-6}
 & Narrative Ending                                                                   & 10.0       & 20.0     &      45.0     &  \textbf{85.0}     \\ \hline\hline
\multirow{3}{*}{Flexibility} & Emotional Flexibility                                                              &   20.0     &  25.0    &    55.0       &  \textbf{90.0}    \\ \cline{2-6}
& Perspective \& Voice Flexibility                                                   &  10.0     &   20.0   &     25.0      &  \textbf{70.0}     \\ \cline{2-6}
& Structural Flexibility                                                             &  15.0      &  30.0    &    35.0       & \textbf{90.0}     \\ \hline\hline
\multirow{3}{*}{Originality} & Originality in Form \& Structure                                                   & 0.0       &   15.0   &     0.0      &  \textbf{60.0}     \\ \cline{2-6}
& Originality in Thought                                                             &   5.0     &   60.0   &     35.0      &  \textbf{90.0}     \\ \cline{2-6}
& Originality in Theme \& Content                                                    &  0.0      &  30.0    &     10.0      &  \textbf{85.0}     \\ \hline\hline
\multirow{3}{*}{Elaboration} &  World Building \& Setting                                                          &   15.0     &   35.0   &    65.0       &  \textbf{90.0}    \\ \cline{2-6}
& Character Development                                                              &   10.0     &  20.0   &  25.0        &  \textbf{75.0}    \\ \cline{2-6}
& Rhetorical Complexity                                                              &    5.0    &  10.0    &    10.0       &  \textbf{90.0}    \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{absolutehumaneval}\textbf{Absolute Evaluation}: Average passing rate on individual creativity test obtained from 8 creative writing experts across all stories in our test set authored by GPT3.5,GPT4,Claude and Humans}

\begin{tabular}{|l|l|l|l|l|}
\hline
                                                                               & GPT3.5 & GPT4 & Claudev1.3 & Human \\ \hline
\begin{tabular}[c]{@{}l@{}}Relative Ranking Based on Preference\end{tabular} & 3.45   & 3.0  & 2.35       & 1.2   \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{relativehumaneval} \textbf{Relative Evaluation}:Average ranking provided by 8 creative writing experts based on their subjective preference across all stories in our test set authored by GPT3.5,GPT4,Claude and Humans}
\end{table*}
